Rethink the Role of Deep Learning towards Large-scale Quantum Systems

Characterizing the ground state properties of quantum systems is fundamental to capturing their behavior but computationally challenging. Recent advances in AI have introduced novel approaches, with diverse machine learning (ML) and deep learning (DL) models proposed for this purpose. However, the necessity and specific role of DL models in these tasks remain unclear, as prior studies often employ varied or impractical quantum resources to construct datasets, resulting in unfair comparisons. To address this, we systematically benchmark DL models against traditional ML approaches across three families of Hamiltonian, scaling up to 127 qubits in three crucial ground-state learning tasks while enforcing equivalent quantum resource usage. Our results reveal that ML models often achieve performance comparable to or even exceeding that of DL approaches across all tasks. Furthermore, a randomization test demonstrates that measurement input features have minimal impact on DL models' prediction performance. These findings challenge the necessity of current DL models in many quantum system learning scenarios and provide valuable insights into their effective utilization.

==> contents/tables/exp1/mqc.tex <==
\begin{table}
    \centering
    \caption{The total number of query complexity under experimental setup, where part of data grids are marked with the same color for the same $M_{\rm{QC}}=n\times M$.}
    \begin{tabular}{c||c|c|c|c}
    \toprule
      {} &$M=$ 64 & 128 & 256 & 512 \\
        \midrule
    $n_{\rm{}}=$20 &{1280} & \cellcolor[HTML]{CB4154}\textcolor{white}{2560} & \cellcolor[HTML]{228B22}\textcolor{white}{5120} & \cellcolor[HTML]{4169E1}\textcolor{white}{10240} \\ 
40 & \cellcolor[HTML]{CB4154}\textcolor{white}{2560} & \cellcolor[HTML]{228B22}\textcolor{white}{5120} & \cellcolor[HTML]{4169E1}\textcolor{white}{10240} & \cellcolor[HTML]{DAA520}{20480} \\
60 & {3840} & {7680} & 15360  & {30720} \\
80 & \cellcolor[HTML]{228B22}\textcolor{white}{5120} & \cellcolor[HTML]{4169E1}\textcolor{white}{10240} & \cellcolor[HTML]{DAA520}{20480} & {40960} \\
100 & {6400} & {12800} & {25600} & {51200} \\
\bottomrule
    \end{tabular}
    \label{tab:query_complexity}
    \vspace{-8pt}
\end{table}

==> contents/tables/exp1/query_complexity.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{c||c|c|c|c}
    \toprule
      {} &$M=$ 64 & 128 & 256 & 512 \\
        \midrule
    $n_{\rm{tr}}=$20 &\cellcolor{red!10}{{1280}} & \cellcolor{red!20}{2560} & \cellcolor{red!30}{5120} & \cellcolor{red!50}{10240} \\ 
40 & \cellcolor{red!20}{2560} & \cellcolor{red!30}{5120} & \cellcolor{red!50}{10240} & \cellcolor{red!70}{20480} \\
60 & \cellcolor{red!30}{3840} & \cellcolor{red!40}{7680} & \cellcolor{red!60}{15360} & \cellcolor{red!80}{30720} \\
80 & \cellcolor{red!30}{5120} & \cellcolor{red!50}{10240} & \cellcolor{red!70}{20480} & \cellcolor{red!90}{40960} \\
100 & \cellcolor{red!40}{6400} & \cellcolor{red!50}{12800} & \cellcolor{red!75}{25600} & \cellcolor{red!100}{51200} \\
\bottomrule
    \end{tabular}
    \caption{The total number of query complexity $M_{QC}$}
    \label{tab:query_complexity}
\end{table}

==> contents/tables/exp2/acc_phase_rydberg.tex <==
\begin{table*}[htp]
            \centering
            \renewcommand{\arraystretch}{1.2} % Adjust row height
            \caption{\small{\textbf{The classification result of quantum phases on the 1-dimensional Rydberg atom model with varied $N$ and $n_{\rm{sft}}$}. $M$ is fixed to $64$. The best results are highlighted in \colorbox{green!40}{\textbf{boldface}} while the second-best results are distinguished in \colorbox{green!20}{\underline{underlined}}. }}
            \vspace{-10pt}
            \resizebox{\linewidth}{!}{
            \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
                \toprule
                \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{$N=16$} &  \multicolumn{3}{c|}{$N=25$}  &  \multicolumn{3}{c}{$N=31$}  \\
        {}& $n_{\rm{sft}}=20$ & $n_{\rm{sft}}=60$ & $n_{\rm{sft}}=100$ & $n_{\rm{sft}}=20$ & $n_{\rm{sft}}=60$ & $n_{\rm{sft}}=100$ &  $n_{\rm{sft}}=20$ & $n_{\rm{sft}}=60$ & $n_{\rm{sft}}=100$ \\
        \midrule
        %Classical shadow & \multicolumn{3}{c|}{$0.21113$} & \multicolumn{3}{c|}{$0.21257$} & \multicolumn{3}{c|}{$0.21399$} & \multicolumn{3}{c}{$0.21447$} \\
        %\hline
        MLP & $91.50$ & $93.14$ & $93.86$ & \cellcolor{green!20}{\underline{$89.00$}} & \cellcolor{green!20}{\underline{$92.36$}} & $89.50$ & $92.43$ & \cellcolor{green!40}{$\bm{92.93}$} & $92.79$ \\
        CNN & $91.71$ & $91.86$ & $92.71$ & $88.86$ & $91.07$ & $91.07$ & $92.42$ & \cellcolor{green!20}{\underline{$92.64$}} & $92.50$  \\
        %Shadow generator & $0.22127$ & $0.20645$  & $0.20391$ & $0.21981$ & $0.22062$ & $0.21066$ & $0.23070$ & $0.20901$ & $0.20575$ \\
        LLM4QPE & $87.29$ & $93.57$ & $94.07$ & $-63.93-$ & $80.43$ & $88.79$ & $61.21-$ & $76.50$ & $85.36$   \\   
        \hline
        %LLM4QPE w/o pretrain  & $0.06848$ & $0.04736$ & $0.02856$ & $0.07262$ & $0.04310$ & $0.03867$ & $0.07268$ & $0.04434$ & $0.03813$ & $0.05080$ & $0.04387$ & $0.02782$  \\
        Dirichlet Kernel & $79.64$ & $80.21$ & $82.43$ & $87.71$ & $86.57$ & $89.14$ & $83.57$ & $90.57$ & $90.21$\\
        RBF Kernel  & $90.64$ & $89.86$ & $90.86$ & $87.07$ & $88.29$ & $88.29$ & ${86.79}$ & \cellcolor{green!40}{$\bm{92.93}$} & $93.29$ \\
        NTK & $91.43$ & \cellcolor{green!20}{\underline{$95.93$}} & $96.00$ & $88.64$ & \cellcolor{green!40}{$\bm{93.29}$} & $93.36$ & $91.64$ & $89.57$ & $93.64$ \\
        KNN & $93.36$ & $92.21$ & $94.29$ & $88.93$ & $92.14$ & $91.86$ & $90.57$ & \cellcolor{green!20}{\underline{$92.64$}} & $92.79$ \\ % K-nearest neighbor
        %Decision Tree & $90.36$ & $94.71$ & $96.36$ & $85.93$ & $85.93$ & $93.57$ & $90.29$ & $91.93$ & $93.21$ \\
        RandomForest & \cellcolor{green!20}{\underline{${94.21}$}} & ${94.21}$ & ${95.43}$ & ${88.21}$ & {${92.00}$} & ${93.07}$ & {$87.71$} & ${91.93}$ & ${92.14}$ \\
        LightGBM & $91.57$ & $93.85$ & $92.36$ & $86.50$ & $91.43$ & \cellcolor{green!20}{\underline{$94.07$}} & $92.93$ & $91.14$ & \cellcolor{green!40}{$\bm{95.64}$} \\
        GradientBoosting & \cellcolor{green!20}{\underline{$94.21$}} & $95.79$ & \cellcolor{green!40}{$\bm{98.07}$} & $88.50$ & $92.29$ & \cellcolor{green!40}{$\bm{94.79}$} & \cellcolor{green!20}{\underline{$93.21$}} & $92.43$ & \cellcolor{green!20}{\underline{$95.14$}} \\
        XGBoost & \cellcolor{green!40}{$\bm{94.36}$} & \cellcolor{green!40}{{$\bm{96.28}$}} & \cellcolor{green!20}{\underline{${96.71}$}} & \cellcolor{green!40}{$\bm{89.07}$} & ${92.07}$ & ${93.71}$ & \cellcolor{green!40}{$\bm{94.21}$} & ${92.36}$ & ${94.43}$ \\
        \bottomrule
      
    \end{tabular}
    }   
    \label{Tab:rydberg_phase_acc}
\end{table*}

==> contents/tables/exp2/rmse_correlation_hei2.tex <==
\begin{table*}[ht]
            \centering
            \caption{The prediction RMSE of two-point correlation function on the two-dimensional Heisenberg model with varied system sizes $n_q$ and sup. training sizes $n_{\rm{tr}}$.}
            \renewcommand{\arraystretch}{1.2} % Adjust row height
            \resizebox{\linewidth}{!}{
            \begin{threeparttable}
            \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
                \toprule
                \multirow{2}{*}{Methods} &  \multicolumn{3}{c|}{$n_q=8\times 5$} &  \multicolumn{3}{c|}{$n_q=9\times 5$}  &  \multicolumn{3}{c|}{$n_q=8\times 8$} & \multicolumn{3}{c}{$n_q=10\times 10$}  \\
        {}& $n_{tr}=20$ & $n_{tr}=50$ & $n_{tr}=90$ & $n_{tr}=20$ & $n_{tr}=50$ & $n_{tr}=90$ &  $n_{tr}=20$ & $n_{tr}=50$ & $n_{tr}=90$ &$n_{tr}=20$ & $n_{tr}=50$ & $n_{tr}=90$\\
        \midrule
        Classical Shadow & \multicolumn{3}{c|}{$0.34233$} & \multicolumn{3}{c|}{$0.$} & \multicolumn{3}{c|}{$0.$} & \multicolumn{3}{c}{$0.40426$}   \\
       Pretrain-SFT  & &  &  &  &  &  & & & & &   \\
       DK$^{2}$ & 0.26226 & 0.25764 & 0.25789 & 0.31372 & 0.31395 & 0.31570 & 0.25411 & 0.26005 & 0.25985 & 0.30747 & 0.30584 & 0.30611\\
       RBF  & 0.29610 & 0.27135 & 0.26345 & 0.33274 & 0.32095 & 0.31866 & 0.28660 & 0.27224 & 0.26523 & 0.31583 & 0.30896 & 0.30731\\
       NTK  & 0.25502 & 0.25331 & 0.25367 & 0.30789 & 0.31031 & 0.31261 & 0.24492 & 0.25497 & 0.25551 & 0.30602 & 0.30471 & 0.30477\\
       MLP & 0.32501 & 0.31099 & 0.31749 & 0.37102 & 0.36356 & 0.36531 & 0.32306 & 0.31763 & 0.32043 & 0.35867 & 0.35470 & 0.35451 \\
       Lasso  & 0.26605 & 0.23510 & 0.22073 & 0.31842 & 0.28941 & 0.27585 & 0.27290 & 0.23958 & 0.22734 & 0.30099 & 0.27847 & 0.26828\\
       Ridge & 0.26224 & 0.25755 & 0.25771 & 0.31370 & 0.31391 & 0.31563 & 0.25408 & 0.25997 & 0.25970 & 0.30747 & 0.30582 & 0.30609 \\
        \bottomrule
      
    \end{tabular}
    \end{threeparttable}}   
    \label{Tab:hei2d_regression_res_correlation}
\end{table*}

==> contents/tables/exp3/is_bigger_often_better.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
        \toprule
      Model & # params & $L_2$ regularization weights  & Performance (RMSE) \\
      \midrule
      Lasso (optimal) & - & - & 0.01117 \\
      MLP-128 dims & 4,145,281 & 954.55 &  0.01258 \\
      MLP-64 dims &2,080,705 &1204.50 & 0.01292 \\
      MLP-32 dims &1,048,417 &1204.50 & 0.01306 \\
      MLP-16 dims & 532,273 & 756.46 & 0.01285 \\ 
      LLM4QPE & 18,135,425 &0.0004 & 0.01618 \\
      \bottomrule
      
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> contents/tables/learning_models.tex <==

\begin{table*}[htp]
            \caption{Learning-based models for QSL problem.}
            \centering
            \begin{tabular}{c|c}
            \toprule
              Type & Model (cite)  \\
              \midrule
               \multirow{5}{*} {Classical machine learning}  & Dirichlet Kernel~\cite{huang2022provably} \\
               {} & Radial Basis Function (RBF) Kernel~\cite{huang2022provably} \\
               {} & Neural Tangent Kernel~\cite{huang2022provably} \\
               {} & $\ell_1$-regularized Regression~\cite{lewis2024improved} \\
               {} & $\ell_2$-regularized Regression \\
               \hline
               \multirow{3}{*}{Deep learning} &   Nerual networks such as Multilayer Perceptron and Convolutional Neural Network\\
               %{} & PixelCNN~\cite{sharir2020deep}\\
               {} & Transformer-based shadow generator~\cite{wang2022predicting} \\
               {} & LLM-like pretrain and SFT paradigm~\cite{tang2024towards} \\
               \bottomrule
            \end{tabular}
            \label{tab:learning_model}
        \end{table*}
